Algebraic Convolutional Filters on Lie Group Algebras

Group convolutional neural networks are a useful tool for utilizing symmetries known to be in a signal; however, they require that the signal is defined on the group itself. Existing approaches either work directly with group signals, or they impose a lifting step with heuristics to compute the convolution which can be computationally costly. Taking an algebraic signal processing perspective, we propose a novel convolutional filter from the Lie group algebra directly, thereby removing the need to lift altogether. Furthermore, we establish stability of the filter by drawing connections to multigraph signal processing. The proposed filter is evaluated on a classification problem on two datasets with $SO(3)$ group symmetries.

==> figures/fig10_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%


%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{180, 222,44}
\definecolor{my_cp5_col3}{RGB}{94, 201, 98}
\definecolor{my_cp5_col4}{RGB}{33, 145, 140}
\definecolor{my_cp5_col5}{RGB}{59, 82, 139}
\definecolor{my_cp5_col6}{RGB}{68, 1, 84}


\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {1*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {1*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
 
\tikzstyle{myboxlabel} = [set,
fill=my_cp5_col3,
minimum width  = 1.61*\unit,
minimum height = 0.5*\unit]
 
 
                             

\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{8}{8}\selectfont	
	
	
\begin{tikzpicture}[scale=\scale,rounded corners,ultra thick]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Color Labels palette  %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


   %%------------ Label 1 --------
   
   \path (0,0) node [] (L1) {};
   \path (L1) ++ (0, 0) node [rotate=90, color=black] {Label 1};
   
   
   %%------------ Label 2 --------
   
    \path (L1.south)++(0,\vertsep) node [] (L2) {};
    \path (L2) ++ (0, 0) node [rotate=90, color=black] {Label 2};
    
    
     %%------------ Label 3 --------
     
     \path (L2.south)++(0,\vertsep) node [] (L3) {};
     \path (L3) ++ (0, 0) node [rotate=90, color=black] {Label 3};  
    
    
     %%------------ Label 4 --------
         
     \path (L3.south)++(0,\vertsep) node [] (L4) {};
     \path (L4) ++ (0, 0) node [rotate=90, color=black] {Label 4}; 
    
 

\end{tikzpicture}


}






